Equivariant Subgraph Aggregation Networks

Message-passing neural networks (MPNNs) are the leading architecture for deep learning on graph-structured data, in large part due to their simplicity and scalability. Unfortunately, it was shown that these architectures are limited in their expressive power. This paper proposes a novel framework called Equivariant Subgraph Aggregation Networks (ESAN) to address this issue. Our main observation is that while two graphs may not be distinguishable by an MPNN, they often contain distinguishable subgraphs. Thus, we propose to represent each graph as a set of subgraphs derived by some predefined policy, and to process it using a suitable equivariant architecture. We develop novel variants of the 1-dimensional Weisfeiler-Leman (1-WL) test for graph isomorphism, and prove lower bounds on the expressiveness of ESAN in terms of these new WL variants. We further prove that our approach increases the expressive power of both MPNNs and more expressive architectures. Moreover, we provide theoretical results that describe how design choices such as the subgraph selection policy and equivariant neural architecture affect our architecture's expressive power. To deal with the increased computational cost, we propose a subgraph sampling scheme, which can be viewed as a stochastic version of our framework. A comprehensive set of experiments on real and synthetic datasets demonstrates that our framework improves the expressive power and overall performance of popular GNN architectures.

==> approach_notes.tex <==
\subsection{Formulation}

Let us consider a graph $G = (V, E)$, with $V$ set of nodes, cardinality $|V| = n$, $E \subseteq V \times V$ set of edges, cardinality $|E| = m$.

For now we could conveniently consider subgraphs of $G$ obtained by taking subsets of the original edge set $E$. This includes disconnected subgraphs and also subgraphs containing isolated nodes. According to this choice, we always retain the original node set $V$ of $G$; while this does not have an impact on the expressive power of the approach (verify), it may turn out to be a particularly convenient practical choice, especially when using DSS aggregators. Alternatively, it would also be possible to redefine the subgraph selection in terms of node subsets and their induced subgraphs.

The powerset $\mathbb{P}(E) = \{ F | F \subseteq E\}$ represents the set of all possible subsets of $E$ and allows us to conveniently express the collection of all possible subgraphs of $G$:
$$
    \mathcal{S}_G = \{(V, F) | F \in \mathbb{P}(E)\}
$$
Interestingly, we notice that $\mathbb{P}(E)$ includes:
\begin{itemize}
    \item the empty (sub)set $F_\bot = \emptyset$
    \item the degenerate subset $F_\top = E$
\end{itemize}
\noindent and that the corresponding subgraphs are of particular distinction: the subgraph $G_\bot = (V, F_\bot)$ is a set (no connectivity), while the subgraph $G_\top = (V, F_\top) = G$ corresponds to the original graph. In general, the presence on the special subgraph $G_\top$ is important to guarantee an expressive power which is at least the one of the employed GNN encoder (see counterexample in Figure~\ref{fig:edge_negative_example}).

Importantly, the cardinality of $\mathcal{S}_G$ grows exponentially with the number of edges $m$: $|\mathcal{S}_G| = 2^{m}$. This raises a natural question: can we retain the full expressive power of the method by considering only a specific selection of subgraphs?

\subsection{Subgraph selection}

A subgraph selection $\mathcal{S}_G^{\pi} \subseteq \mathcal{S}_G$ corresponds to a subset of the overall set of subgraphs, chosen according to a specific policy $\pi$.

Subgraph selection policies may include, for example:
\begin{itemize}
    \item Removing one node
    \item Removing one edge
    \item Spanning trees
    \item Egonets of certain sizes (e.g. all depth 1 egonets, all depth 2 egonets)
    \item Adding node features and/or edge features in an invariant way (i.e. so that the mapping from $G \mapsto \mathcal{S}_G^\pi$ is invariant to node permutations on $G$.)
\end{itemize}

Importantly, the choice of the selection policy may have an impact the equivariance/invariance properties of the overall model. For example, if the the subset selection $\mathcal{S}_G^{\pi_a} = \big\{ ( V, E \backslash \{ (i, j) \} ) | (i, j) \in E \big\}$ guarantees node permutation equivariance/invariance, the selection $\mathcal{S}_G^{\pi_b} = \big\{ ( V, E \backslash \{ (1, j) \} ) | (1, j) \in E \big\}$ does not – as it explicitly depends on the ordering of the nodes.

Notice how two particular selection policies allow us to directly relate our method to reconstruction conjectures. In particular, the policy $\pi_c$ such that we select all possible node-deleted subgraphs generates a selection $\mathcal{S}_G^{\pi_c}$ which is the \emph{deck} of graph $G$, according to the (standard) Reconstruction Conjecture. The policy $\pi_a$, such that we select all possible edge-deleted subgraphs, generates $\mathcal{S}_G^{\pi_a}$: the \emph{edge-deck} of graph $G$ according to the Edge Reconstruction Conjecture.

\todo[inline]{FF: Here we should introduce the conjectures more formally and also explain what is their impact in terms of model expressivity}

\subsection{Architectures.} We discussed two possible architectures: (1) DS-GNN: Siamese MPNN followed by deepsets applied to the invariant subgraph representations  (2)DSS-GNN: use DSS layers in which the equivariant inner layers are MPNNs.

Here a more formal description follows. We denote as $\mathcal{G} = \{ G_1, \mathellipsis G_n \} = \{ G_i \}_{i=1}^{n}$ the set of $n$ graphs in input to the proposed architecture. This can be obtained, for example, by applying any subgraph selection policy $\pi$ to an input graph $G$, such that $\mathcal{G} = \mathcal{S}^{\pi}_G$. 

\paragraph{DS-GNN.} TBA.

\paragraph{DSS-GNN.} The DSS-GNN model has the following layer structure:
\begin{equation}\label{eq:dssgnn_layer_structure}
    L(\mathcal{G})_i = L_1(A_i,X_i) + L_2(\sum_{j=1}^n A_j, \sum_{j=1}^n X_j)
\end{equation}
where $A_i,X_i$ are the adjacency and node feature matrices of graph $G_i$ and $L_1, L_2$ are MPNNs. We note that the summation aggregation function can be replaced by max or mean, or even by an attention module. When graphs are obtained via edge-deletion selection policy on an (unweighted) input graph $G$, it may also be convenient to define the aggregation on adjacency matrices as $\frac{1}{n-1} \sum_{j=1}^n A_j$, which recovers $G$'s original connectivity.

MPNNs can be parameterised, for example, according to the formulation due to \cite{morris2019weisfeiler}, which updates the representation of node $\ell$ as:
$$
    L_k(A, X)_\ell = W^k_1 X_\ell + W^k_2 \sum_{m \sim_A \ell} X_m
$$
\noindent where $k=1, 2$, $\sim_A$ denotes the neighboring relation induced by matrix $A$ and $X_\ell, X_m$ represent the feature vectors for nodes $\ell, m$ respectively.

Combining the last two equations, we obtain the following equation which describes how the model updates the representation node $\ell$ in graph $G_i$:
\begin{equation}\label{eq:linear_dssgnn}
    L(\mathcal{G})_{i,\ell} = W^1_1 X_{i,\ell} + W^1_2 \sum_{m \sim_i \ell} X_{i, m} + W^2_1 \sum _{j=1}^n X_{j,\ell} + W^2_2 \sum_{m \sim \ell} \sum_{j=1}^n X_{j,m}
\end{equation}
\noindent where we have generally denoted as $\sim_i$ the neighboring relation induced by adjacency matrix $A_i$, and by $\sim$ the one induced their aggregation.

A `deep', equivariant, non-linear model is obtained by stacking multiple such layers interspersed by non-linear activations $\sigma$: $\mathcal{M} = \sigma \circ L^T \circ \sigma \circ \mathellipsis \circ \sigma \circ L^1$.

The proposed architecture is very general. As we show in the following, it can implement a variety of operations on the set of graphs in input.

\begin{proposition}\label{prop:dssgnn_implements_ds}
    A DSS-GNN architecture with $T \geq 4$ layers in the form of equation~\ref{eq:linear_dssgnn} can implement a node-wise DeepSets~\citep{zaheer2017deep} model over the set of node representations on each input graph in $\mathcal{G}$. Such a model is invariant w.r.t. the order of graphs in $\mathcal{G}$.
\end{proposition}
\begin{proof}
    According to~\citet{zaheer2017deep}, any permutation invariant function $f(X)$ operating on a set $X$ \emph{of elements from a countable universe}
    \todo[inline]{FF: discuss the conditions on X}
    is decomposable as $f(X) = \rho \big( \sum_{x \in X} \phi (x) \big)$ for suitable mappings $\rho, \phi$. In practice, these can be replaced by universal function approximators such as Multi Layer Perceptrons (MLPs).

    Let $X = \{ h_{v,i} | i = 1, \mathellipsis, n \}$ be the set of node representations for each graph $G_i \in \mathcal{G}$. In order to prove the proposition it is sufficient to describe a DSS-GNN, say $\mathcal{M}$, which satisfies the hypothesis and implements such $f$ function as described above.
    
    Such a model is obtained by stacking two components: $\mathcal{M} = \mathcal{M}_\rho \circ \mathcal{M}_\phi$. The first component, $\mathcal{M}_\phi$ effectively implements an MLP applied independently on each $h_{v,i}$ and is obtained as $\mathcal{M}_\phi = \sigma \circ L_{T_\phi} \circ \sigma \circ \mathellipsis \circ \sigma \circ L_{1}, T_\phi \geq 1$. Here, $L$ represent a DSS-GNN layer where $W_2^1, W_1^2, W_2^2 = \mathbf{0}$.
    
    The second component is obtained as $\mathcal{M}_\rho = L_{T_\rho} \circ \sigma \circ \mathellipsis \circ \sigma \circ L_{1}, T_\rho \geq 3$. Here, any $L$ is a DSS-GNN layer. In particular, $L_1$ is such that $W_1^1, W_2^1, W_1^2 = \mathbf{0}$ and any other layer $L_t$, $t = 2, \mathellipsis, T_\rho$ is such that $W_1^1, W_2^1, W_2^2 = \mathbf{0}$.
\end{proof}

\begin{proposition}\label{prop:dssgnn_implements_gnn}
    A DSS-GNN architecture with $T \geq 1$ layers in the form of equation~\ref{eq:linear_dssgnn} can implement a $T$-layer MPNN model in the form of~\citep{morris2019weisfeiler} independently applied to each of the graphs in $\mathcal{G}$. Such a model is equivariant w.r.t. to the order of nodes in each graph from $\mathcal{G}$.
\end{proposition}
\begin{proof}
    Such a DSS-GNN model can be described as $\mathcal{M} = \sigma \circ L_{T} \circ \sigma \circ \mathellipsis \circ \sigma \circ L_{1}$. Here $L_t, t = 1, \mathellipsis, T$ is a DSS-GNN layer where $W_1^2, W_2^2 = \mathbf{0}$.
\end{proof}

\begin{proposition}\label{prop:dssgnn_implements_ds_gnn}
    Let $T = T_s + 1, T_s \geq 4$. A DSS-GNN architecture with $T$ layers in the form of equation~\ref{eq:linear_dssgnn} can implement an equivariant MPNN layer in the form of~\citep{morris2019weisfeiler} applied to the graph whose: (i) connectivity is given by the union of the topologies of graphs in $\mathcal{G}$; (ii) node features result from any cross-graph node-wise permutation invariant function that can be expressed by a $T_s$-layer DeepSets model.
\end{proposition}
\begin{proof}
    Such a DSS-GNN model can be described as $\mathcal{M} = L_g \circ \mathcal{M}_s$. Here $\mathcal{M}_s$ is a $T_s$-layer DSS-GNN model satisfying Proposition~\ref{prop:dssgnn_implements_ds} and $L_g$ is a DSS-GNN layer where $W_1^1, W_2^1 = \mathbf{0}$.
    \todo[inline]{FF: in input to Lg I may need to rescale the node features from each of the graphs: they are all equal and represent the needle-colours, but are summed all together again. I guess I can simply make use of W matrices for that? Note: Forcing the aggregation to generally be "mean" may decrease the expressive power in case we work with multisets, so probably not a great choice.}
\end{proof}




\subsection{Known instantiations}

Our framework captures several previously existing models, with proper choices of subgraph policies $S_G^\pi$ and symmetry groups $H$.

\textbf{Relational Pooling} \citep{murphy2019relational}: take $S_G^{\pi} = \{(G, [X; p \cdot I] : p \in S_n \}$. 
If the base function $\vec f$ is a GNN, then we take $H$ to be the standard group that acts by permuting node ids of subgraphs. If $\vec f$ is a generic function, we take $H$ to be the trivial group.
This means that the set of subgraphs is of size $n!$, and is given by repeating the same combinatorial graph $G$, but appending each permutation $p \cdot I$ of the identity matrix as node features to some subgraph.

Our model can also express a k-ary RP in \citep{murphy2019relational}, which operates on all induced subgraphs on $k$ nodes of $G$. In this case, we take $S_G^{\pi}$ to be all $k$-node induced subgraphs of $G$. The symmetry group $H$ is taken similarly to the above.

We can also express a form of the local relational pooling of \cite{zhengdao2020can} by taking $S_G^\pi$ to be the depth $l$ egonets of $G$ in all possible permutations.

\textbf{Identity Aware GNN} \citep{you2021identity}: take $S_G^\pi$ to be all depth $K$ egonets of $G$, and add a node feature dimension that is $1$ for the center node of the egonet, and $0$ for all other nodes. There are $|S_G^\pi| = n$ subgraphs in this case.

\textbf{Structural Message Passing} \citep{vignac2020building}: take $S_G^\pi$ to be $n$ copies of the same combinatorial $G$, with node features for subgraph $i$ to be $U_i \in \mathbb{R}^{n \times d+1}$, where $U_i[i,:] = [1; x_i]$ for the original node features $x_i$ of node $i$, and $U_i[j,:] = 0$ for $j \neq i$. The symmetry group is $S_n$, where it permutes both rows and columns of the node feature tensor $\mathbf{U} = [U_1, \ldots, U_n] \in \mathbb{R}^{n \times n \times d+1}$, as well as both rows and columns of the adjacency $\mA$.

\textbf{Adding node features}: for any other approach that adds node features (e.g adding random node features as in \cite{sato2021random}, random colorings as in \cite{dasoulas2019coloring}), we can have $S_G^\pi$ to be any number of copies of the same combinatorial $G$ with a sampling of node features. For random node features, our mapping from $G \mapsto S_G^\pi$ will no longer be exactly invariant, but it will be invariant in expectation. In the random node features case, we can sample node features $k$ times if $|S_G^\pi| = k$. Then if the DeepSets / subgraph aggregation is a mean, we approximate the expectation over the random node feature distribution.

\textbf{DropEdge} \citep{rong2019dropedge}: take a stochastic policy that forms subgraphs that randomly drop some edges from the original graph. DropEdge can thus be seen as a stochastic approximation for our method when taking subgraphs from deleting multiple edges.

\textbf{Adding Nodes and Edges}: Given a graph $G$, we can augment with versions of the graph where we add nodes and edges in an invariant way. For instance, we can have the policy be $S_G^\pi = \{G, K_n\}$ where $K_n$ is the complete graph on $n$ vertices; this combined with DSS updates allow us to generalize fully adjacent (FA) layers \cite{alon2021bottleneck} and global readouts in node updates in ACR-GNN \cite{barcelo2020logical}. 

==> ogb_sampling.tex <==
\begin{table}[ht]
\centering
\scriptsize
 \caption{Results of our stochastic sampling approach on OGB datasets, where each graph sees $100\%, 50\%, 20\%, 5\%$ of the  subgraphs in the selected policy.  Gray background indicates that ESAN outperforms the base encoder.}
\label{tab:ogb_datasets_sampling}
    \begin{tabular}{ll |l l} %
    \toprule
    &  & 
    \textsc{ogbg-molhiv} &
    \textsc{ogbg-moltox21} \\
     & & \textbf{ROC-AUC (\%)} & \textbf{ ROC-AUC (\%)}\\
    \midrule       


    \textsc{GIN}~\citep{xu2018how}  & &
    75.58$\pm$1.40 &
    74.91$\pm$0.51
    \\
    \midrule


    \multirow{4}{*}{\bf \textsc{DS-GNN (GIN) (ED)}}  & {\bf \textsc{100\%}} & 
    \cellcolor{Gray}76.43$\pm$2.12&
    \cellcolor{Gray}75.12$\pm$0.50\\

    &{\bf \textsc{50\%}}   & 
    \cellcolor{Gray}76.29$\pm$1.33& 
    74.59$\pm$0.71\\

    &{\bf \textsc{20\%}}   & 
    \cellcolor{Gray}76.57$\pm$1.48&
    \cellcolor{Gray}75.67$\pm$0.89\\

    &{\bf \textsc{5\%}}   & 
    \cellcolor{Gray}77.82$\pm$1.0&
    \cellcolor{Gray}76.39$\pm$1.11\\
    \midrule


    \multirow{4}{*}{\bf \textsc{DS-GNN (GIN) (ND)}}  & {\bf \textsc{100\%}} & 
    \cellcolor{Gray}76.19$\pm$0.96&
    \cellcolor{Gray}75.34$\pm$1.21\\

    &{\bf \textsc{50\%}}   & 
    \cellcolor{Gray}77.23$\pm$1.32&
    74.82$\pm$1.05\\

    &{\bf \textsc{20\%}}   & 
    \cellcolor{Gray}77.65$\pm$0.84&
    \cellcolor{Gray}75.66$\pm$0.46\\

    &{\bf \textsc{5\%}}   & 
    \cellcolor{Gray}78.26$\pm$1.02&
    \cellcolor{Gray}76.51$\pm$1.04\\
    \midrule


    \multirow{4}{*}{\bf \textsc{DS-GNN (GIN) (EGO)}}  & {\bf \textsc{100\%}} &
    \cellcolor{Gray}78.00$\pm$1.42&
    \cellcolor{Gray}76.22$\pm$0.62\\

    &{\bf \textsc{50\%}}   & 
    \cellcolor{Gray}76.52$\pm$0.72&
    \cellcolor{Gray}75.98$\pm$0.72\\

    &{\bf \textsc{20\%}}   & 
    \cellcolor{Gray}77.49$\pm$1.32&
    \cellcolor{Gray}75.88$\pm$0.5\\

    &{\bf \textsc{5\%}}   & 
 73.92$\pm$1.78&
    \cellcolor{Gray}74.95$\pm$0.54\\
    \midrule

    \multirow{4}{*}{\bf \textsc{DS-GNN (GIN) (EGO+)}}  & {\bf \textsc{100\%}} &
    \cellcolor{Gray}77.40$\pm$2.19&
    \cellcolor{Gray}76.39$\pm$1.18
    \\

    &{\bf \textsc{50\%}}   & 
    \cellcolor{Gray}76.91$\pm$1.22&
    \cellcolor{Gray}75.69$\pm$1.17\\

    &{\bf \textsc{20\%}}   & 
    \cellcolor{Gray}75.92$\pm$1.59&
    \cellcolor{Gray}75.84$\pm$0.63\\

    &{\bf \textsc{5\%}}   & 
    73.46$\pm$1.8&
    \cellcolor{Gray}75.08$\pm$0.96\\
    \midrule


    \multirow{4}{*}{\bf \textsc{DSS-GNN (GIN) (ED)}}  & {\bf \textsc{100\%}} & 
    \cellcolor{Gray}77.03$\pm$1.81&
    \cellcolor{Gray}76.71$\pm$0.67 \\

    &{\bf \textsc{50\%}}   & 
    \cellcolor{Gray}77.50$\pm$1.82&
    \cellcolor{Gray}76.40$\pm$0.84\\

    &{\bf \textsc{20\%}}   & 
    \cellcolor{Gray}76.82$\pm$1.83&
    \cellcolor{Gray}76.31$\pm$0.90\\

    &{\bf \textsc{5\%}}   & 
    \cellcolor{Gray}76.71$\pm$1.46&
    \cellcolor{Gray}76.84$\pm$0.54\\


    \midrule


    \multirow{4}{*}{\bf \textsc{DSS-GNN (GIN) (ND)}}  & {\bf \textsc{100\%}} & 
    \cellcolor{Gray}76.63$\pm$1.52&
    \cellcolor{Gray}77.21$\pm$0.70
    \\

    &{\bf \textsc{50\%}}   & 
    \cellcolor{Gray}76.96$\pm$1.71&
    \cellcolor{Gray}76.92$\pm$0.94\\

    &{\bf \textsc{20\%}}   & 
    \cellcolor{Gray}76.23$\pm$1.48&
    \cellcolor{Gray}77.07$\pm$1.03\\

    &{\bf \textsc{5\%}}   & 
    \cellcolor{Gray}76.74$\pm$1.67&
    \cellcolor{Gray}76.54$\pm$0.86\\

    \midrule


    \multirow{4}{*}{\bf \textsc{DSS-GNN (GIN) (EGO)}}  & {\bf \textsc{100\%}} &
    \cellcolor{Gray}77.19$\pm$1.27&
    \cellcolor{Gray}77.45$\pm$0.41
    \\

    &{\bf \textsc{50\%}}   & 
    \cellcolor{Gray}76.42$\pm$1.38&
    \cellcolor{Gray}76.37$\pm$1.02\\

    &{\bf \textsc{20\%}}   & 
    \cellcolor{Gray}76.41$\pm$1.05&
    \cellcolor{Gray}77.47$\pm$0.65\\

    &{\bf \textsc{5\%}}   & 
    \cellcolor{Gray}76.38$\pm$1.48&
    \cellcolor{Gray}77.4$\pm$0.58\\

    \midrule

    \multirow{4}{*}{\bf \textsc{DSS-GNN (GIN) (EGO+)}}  & {\bf \textsc{100\%}} &
    \cellcolor{Gray}76.78$\pm$1.66&
    \cellcolor{Gray}77.95$\pm$0.40
    \\

    &{\bf \textsc{50\%}}   & 
    \cellcolor{Gray}76.88$\pm$0.93&
    \cellcolor{Gray}76.42$\pm$0.93\\

    &{\bf \textsc{20\%}}   & 
    \cellcolor{Gray}76.93$\pm$1.45&
    \cellcolor{Gray}76.45$\pm$0.81\\

    &{\bf \textsc{5\%}}   & 
    \cellcolor{Gray}75.97$\pm$0.80&
    \cellcolor{Gray}76.70$\pm$0.56\\

    \bottomrule

    \end{tabular}
\end{table}



==> theory_notes.tex <==
\subsection{Current status}
What can we currently prove? (and have to prove formally) \todo[inline]{HM: Check me please}
\begin{enumerate}
    \item DS,DSS $>$ 1-WL if the original graph is a part taken as one of the subgraphs
    \item for some selection policies like node and edge deletion, DSS$>$1-WL without having to add the original graph since we can reconstruct the original graph
    \item There is a pair of graphs that DS (edges) can separate but DS (nodes) cannot and vice versa (but only 3 edge graphs, edge reconstruction conjecture only considers $\geq$ 4 edges).
    \item DSS(edges) can separate non isomorphic edges that DS(edges cannot)
    \item DS can implement card WL, while DSS can implement deck WL.
    \item distinguishing circular link graphs
\end{enumerate}


\subsection{Examples}


For the case of edge-deleted subgraphs, we want to restrict to graphs of at least 4 edges. See Figure~\ref{fig:edge_negative_example} for a small negative example. This restriction to graphs of at least 4 edges is also done when studying the reconstruction conjecture for edge-deleted subgraphs.

\begin{figure}[ht]
    \centering
    \includegraphics[width=.5\columnwidth]{figures/edge_negative_example.png}
    \caption{Example of two graphs that are non-isomorphic (and can be distinguished by 1-WL) that have the same multiset of edge-deleted subgraphs.}
    \label{fig:edge_negative_example}
\end{figure}

\begin{figure}[ht]
    \centering
    \begin{tabular}{ccc}
         & 
    \subfloat[Original graphs]{\includegraphics[width=.25\columnwidth]{figures/graphs1.pdf}} \hspace{10pt}
    & \\
    \subfloat[Node-deleted subgraphs]{\includegraphics[width=.25\columnwidth]{figures/graphs1_node.pdf}} \hspace{10pt} &
    \subfloat[Edge-deleted subgraphs]{\includegraphics[width=.25\columnwidth]{figures/graphs1_edge.pdf}} \hspace{10pt} &
    \subfloat[Depth 1 egonets]{\includegraphics[width=.25\columnwidth]{figures/graphs1_egonet.pdf}}
    \end{tabular}
    \caption{Two regular graphs that cannot be distinguished by 1-WL, but have multisets of node-deleted subgraphs, edge-deleted subgraphs, and depth-1 egonets that can be distinguished by 1-WL followed by DeepSets.}
    \label{fig:regular1}
\end{figure}



\subsection{Universal Graph Network Case}

The case of universal (permutation equivariant) graph networks is trivial for practice (since we can always add the original graph to the set of subgraphs processed), but it illustrates a difference between DSS and Siamese + DeepSets. DSS with universal graph networks on node-deleted subgraphs of number of nodes $n \geq 3$ is universal, but Siamese + DeepSets on node-deleted subgraphs of number of nodes $n \geq 3$ is universal if and only if the node reconstruction conjecture holds.

This difference in power is because DSS can always reconstruct the original graph (due to maintaining node ordering), while Siamese + DeepSets cannot. Let $\mA$ be the adjacency of the original graph, and $\mA_{-v}$ be the adjacency with all edges to node $v$ deleted. Then $\frac{1}{n-2}\sum_{v \in V} \mA_{-v} = \mA$, so DSS can use the universal graph network to distinguish the original graph $\mA$ from any non-isomorphic graph.

\todo[inline]{Chen: We can say something slightly stronger here. For any subgraph selection policy $\pi$, as long as any edge $e\in E $ of original graph $G$ appear in at least one of the subgraphs $S^{\pi}_G$, we can reconstruct original adjacency matrix $\mA=\sigma(\sum_{g\in S^{\pi}_G} A_g)$, where $\sigma$ applies entry wise on the sum of adjacency matrices. One example is the set of spanning trees. If $G$ is two complete graphs jointed by an ``bridge edge'', the bridge edge will appear in every subgraphs while any other edges of $G$ will not. Therefore, the original adjacency matrix can not be recovered by the formula (linear in $A_g$) in the last paragraph but can be recovered by the one in the current paragraph. (nonlinear in $A_g$). By evoking the universality of graph neural nets, we can then extend the statement from node/edge deleted subgraphs to spanning trees/egonets. 

}

\todo[inline]{An interesting question is that whether there exists a well-defined subgraph selection policy under which one of the edge $e\in G$ does not appear in ALL $S^{\pi}_G$? The answer is yes. Again still consider the two complete graphs joined by an edge. A subgraph selection policy of the following form can exclude the ``bridge edge'': take a egographs within diffusion distance $r$. Note policy certainly does not depends on the node order. By carefully selects the $r$, bridge edge can be excluded in all subgraphs, therefore there is no way we can recover the original graph $G$ from subgraphs $S^{\pi}_G$.}

\subsection {DS vs. DSS}

It may be interesting to investigate additional properties that would make DSS more appealing w.r.t.\ DS. For now, we only have some open questions:
\begin{enumerate}
    \item Would DSS benefit from a better inductive bias and therefore better sample efficiency?
    \item Can DSS afford to use an average smaller number of cards in a graph deck in order to reconstruct it? (NB: This may not necessarily be in contrast with the Reconstruction Conjecture since a DSS-like approach would actually perform different operations! that is, it cannot simply be reduced as "Universally represent each subgraph, \emph{then} universally represent the multiset of their representations.")
    \item Would DSS distinguish different graphs with fewer message passing operations? 
    \item In terms of graph isomorphism testing, can DSS attain better expressive power than DS when using non-universal graph networks / encoders? \todo[inline]{FF: can we relate this last point to the observation above?}
\end{enumerate}

\subsection{A WL perspective (WIP, not formal)}

In this subsection we attempt to formalise our (learnable) graph representation procedures in terms of generalised colour refinement algorithms inspired -- or based on -- the WL test. The hope is that this would allows us to more easily work out some theorical results on the expressive power of our approach, and to appreciate possible inherent theoretical differences between the ``DSS" and ``Siamese+DS" design schemes.

\paragraph{Cards and Decks}

It is convenient here to work in the Edge Reconstruction Conjecture regime, that is to consider the subgraph selection $\mathcal{S}_G$ corresponding to the multiset of edge-deleted subgraphs. In accordance to the typical conjecture terminology, $\mathcal{S}_G$ is termed as $G$'s \emph{deck}\footnote{Technically, we should use the term \emph{edge-deck} in order to distinguish it from the deck generated by node-deletions in the Reconstruction Conjecture.}, whose \emph{cards} are the edge-deleted subgraphs in $\mathcal{S}_G$. It is important to remark that, according to the conjecture, the deck represents a multiset, that is, it may contain multiple copies of the same card. This is due to the fact the different edge-deletions may give birth to the isomorphic subgraphs. For a graphs $G$ with $n$ nodes and $m$ edges, its deck always contains $m$ cards ($|\mathcal{S}_G| = m$), while each card represents a subgraph with $n$, possibly isolated, nodes. The conjecture asserts that any two graphs with at least four edges with the same decks are isomorphic. Notation-wise, we use $G^k$ to refer to the $k$-th card in the deck, and $v_i^k$ for the $i$-th node in card $G^k$.

\paragraph{Card-WL}
We now define the \texttt{Card-WL} algorithm as a generalisation of the standard \texttt{WL} colour refining procedure. Given an input graph $G$, \texttt{Card-WL} works as follows:
\begin{enumerate}
    \item[1)] (\emph{Initialisation}) Construct deck $\mathcal{S}_G$ by all possible single edge-deletions and assign a constant colour $\bar{c}$ to each node for each card in the deck
    \item[2)] (\emph{Color Refinement}) Independently run the \texttt{WL} color refinement step on each card
    \item[3)] Repeat step 2) until convergence on all cards
    \item[4)] (\emph{Card Readout}) Independently compute card-wise colours as $c^{k} = \mathrm{HASH}(\ldblbrace c_i^{k} | i = 1, \mathellipsis, n \rdblbrace), k = 1, \mathellipsis, m$
    \item[5)] (\emph{Readout}) Take $G$'s representation as the multiset of such card-wise colours or, alternatively, compute it as $c^{G} = \mathrm{HASH}(\ldblbrace c^{k} | k = 1, \mathellipsis, m \rdblbrace)$
\end{enumerate}
We already know that this procedure is \textbf{\emph{not less expressive}}\todo[inline]{HM: the term not less expressive is not the correct one here. the two approaches, without adding the original graph, might not be comparable}
 than the standard \texttt{WL} on the original graph $G$ (we do have an exemplary pair undistinguished \texttt{WL} that are distinguished by \texttt{Card-WL}). We are yet to prove that all pairs distinguished by \texttt{WL} are distinguished by \texttt{Card-WL} as well. However, by augmenting deck $\mathcal{S}_G$ with the subgraph $G_\top = G$, it should be easy to show that \texttt{Card-WL} refines \texttt{WL}. 
\todo[inline]{FF: We should prove this formally.}
We remark that the card-wise colours generated at step 4) form a multiset -- and not a set -- due to two reasons:
\begin{enumerate}
    \item[1)] The edge-deletion policy may generate isomorphic subgraphs;
    \item[2)] The edge-deletion policy may generate (possibly non-isomorphic) \texttt{WL}-equivalent subgraphs.
\end{enumerate}
A ``Siamese+DS'' architecture represents the learnable counterpart of the \texttt{Card-WL} procedure, where the Siamese module can be parameterised by means of a \texttt{WL}-equivalent Graph Neural Network such as GIN.

\paragraph{Deck-WL}
\texttt{Deck-WL} differs from \texttt{Card-WL} in the way the readout operations are performed. After the independent application of \texttt{WL} on each card, we first pool node colours across cards, and then represent the original graph based on these ones:
\begin{enumerate}
    \item[1)] Perform steps 1), 2), 3) of \texttt{Card-WL}
    \item[2)] (\emph{Node Readout}) Assign, to each node $v_{i} \in V$, a colour $c_{i}$ according to: $c_{i} = \mathrm{HASH}(\ldblbrace c_{i}^{k} |  k = 1, \mathellipsis, m \rdblbrace)$
    \item[3)] (\emph{Readout}) Take $G$'s representation as the multiset of such node-wise colours or, alternatively, compute it as $c^{G} = \mathrm{HASH}(\ldblbrace c_{i} | i = 1, \mathellipsis, n \rdblbrace)$
\end{enumerate}
A single-layer ``DSS'' architecture may represents the learnable counterpart of \texttt{Deck-WL}. 
\todo[inline]{HM: additional color refinement on the original graph is required.}
\paragraph{Needle-WL}
We notice that the \emph{Node Readout} operation of \texttt{Deck-WL} determines, for each node, an additional multiset of colours that can be employed to augment the \texttt{WL} colour refinement step. Accordingly, we define the \texttt{Needle-WL} algorithm as follows:
\begin{enumerate}
    \item[1)] (\emph{Initialisation}) Construct deck $\mathcal{S}_G$ by all possible single edge-deletions and assign a constant colour $\bar{c}$ to each node for each card in the deck
    \item[2)] (\emph{Color Refinement}) For any $i$, $k$, refine colour $c_{i}^{k}$ as: $c_{i}^{k} \gets \mathrm{HASH}(c_i^{k}, N_i^{k}, C_i)$
    \item[3)] Repeat step 2) until convergence on all cards
    \item[4)] Perform \emph{Node Readout} and \emph{Readout} operations as in \texttt{Deck-WL} (note: \emph{Node Readout} node corresponds to taking $c_{i} = \mathrm{HASH}(C_{i}), i=1, \mathellipsis, n$).
\end{enumerate}
Here, $N_i^{k} =  \ldblbrace c_j^{k} | j \in \mathcal{N}^k(i) \rdblbrace$ and $C_i^{k} =  \ldblbrace c_i^{h} | h = 1, \mathellipsis, m \rdblbrace$. The former term is the multiset of colours of $i$'s neighbours in card $k$, while the latter term is the multiset of $i$'s colours across all other cards in the deck.
\todo[inline]{FF: does the algorithm actually converges !?} 
\todo[inline]{HM: did you check convergence experimentally? proving should be similar the the original proof of convergence of WL ?} 

\todo[inline]{FF: what is the impact of excluding $h = k$ in $C_i^{k}$ ?}

\paragraph{DSS-WL}
We finally introduce the last, most general, variant, which we call \texttt{DSS-WL}. Such a variant works similarly to \texttt{Needle-WL}, with the only difference given by the inclusion of an additional input in the colour refinement step:
\begin{enumerate}
    \item[1)] (\emph{Initialisation}) Construct deck $\mathcal{S}_G$ by all possible single edge-deletions and assign a constant colour $\bar{c}$ to each node for each card in the deck
    \item[2)] (\emph{Color Refinement}) For any $i$, $k$, refine colour $c_{i}^{k}$ as: $c_{i}^{k} \gets \mathrm{HASH}(c_i^{k}, N_i^{k}, C_i, M_i)$
    \item[3)] Repeat step 2) until convergence on all cards
    \item[4)] Perform \emph{Node Readout} and \emph{Readout} operations as in \texttt{Deck-WL}
\end{enumerate}
Here, $M_i = \ldblbrace C_j | j \in \mathcal{N}(i) \rdblbrace$, and aggregates node colours according to the original neighborhoods, i.e. respecting the connectivity induced by the input graph. A multilayer DSS-GNN architecture represents the learnable counterpart of \texttt{DSS-WL}: it is easy to observe the resemblance between the colour refinement step and Equation~\ref{eq:linear_dssgnn}. In particular, when working with the complete set of edge-deleted subgraphs, ${\Sigma A_i}$ in Equation~\ref{eq:linear_dssgnn} recovers $i$'s original neighborhood $\mathcal{N}(i)$, in turn employed in \texttt{DSS-WL} to define input $M_i$. The ability to match the same node across different cards corresponds to a form of graph ``alignment'' which may allow us to increase the expressive power of the model without sacrificing the equivariance/invariance properties of the network.

\paragraph{Cross-card colouring} The inclusion of multisets $C_i^{k}$ induces a form of cross-card colouring, whereby each node refines its colour based on its corresponding colours in the other cards. The observation which intuitively motivates this additional form of colour refinement is that the same node can be coloured differently in different cards, already after the first refinement step (where the update is purely driven by the degree of the node in a specific card\footnote{It is easy to show that this holds also for \texttt{Needle-WL}}). Additionally, it is interesting to notice that this holds true also across isomorphic subgraphs, where the same node may have different degrees and would, more in general, be assigned different colours by a standard run of \texttt{WL}. It is this observation which lead us to hypothesise that \texttt{Needle-WL} may refine \texttt{Card-WL}. It is also reasonable to suppose that, if not more expressive, the former may be able to distinguish non-isomorphic graphs with fewer iterations than the latter.

Next:
\begin{enumerate}
    \item How does \texttt{Deck-WL} generalise standard \texttt{WL}?
\end{enumerate}

\subsection{Expressive Power}





\begin{proposition}\label{prop:ref_implication}
	Let $c, d: S \rightarrow \mathbb{N}$ be colouring functions assigning to each element of $S$ a natural number representing a ``colour'': $c: s \mapsto c_s, d: s \mapsto d_s$.
	Let $A, B$ be two subsets of $S$ and $\mathcal{A}_{\phi}, \mathcal{B}_{\phi}$ be multisets of colours defined as:
	$$
		\mathcal{A}_{\phi} = \ldblbrace \phi_a | a \in A \rdblbrace, \mathcal{B}_{\phi} = \ldblbrace \phi_b | b \in B \rdblbrace, \phi \in \{c, d\}
	$$
	Suppose that $\forall a, b \in A \cup B, d_a = d_b \implies c_a = c_b$ (we write $d \sqsubseteq_{A,B} c$).%
	Then $\mathcal{A}_{c} \neq \mathcal{B}_{c} \implies \mathcal{A}_{d} \neq \mathcal{B}_{d}$.
\end{proposition}
\begin{proof}
	If $\mathcal{A}_{c} \neq \mathcal{B}_{c}$, we assume, w.l.o.g., that there is a colour $\bar{c}$ which is represented more in $\mathcal{A}_{c}$ than in $\mathcal{B}_{c}$. In other words, if we define the two sets:
	$$
		A^{\bar{c}} = \{ a \in A | c_a = \bar{c} \}, B^{\bar{c}} = \{ b \in B | c_b = \bar{c} \}
	$$
	\noindent then $|A^{\bar{c}}| > |B^{\bar{c}}|$. These sets naturally define the partitioning:
	$$
		A = A^{\bar{c}} \cup \tilde{A}^{\bar{c}}, B = B^{\bar{c}} \cup \tilde{B}^{\bar{c}}
	$$
	\noindent where $\tilde{A}^{\bar{c}} = \{ a \in A | c_a \neq \bar{c} \}, \tilde{B}^{\bar{c}} = \{ b \in B | c_b \neq \bar{c} \}$.
	Let us now consider the multisets:
	$$
		\mathcal{A}_d^{*} = \ldblbrace d_a | a \in A^{\bar{c}} \rdblbrace,
		\mathcal{B}_d^{*} = \ldblbrace d_b | b \in B^{\bar{c}} \rdblbrace
	$$
	First, each of these multisets have the same cardinality of the generating sets, that is $|\mathcal{A}_d^{*}| = |A^{\bar{c}}|, |\mathcal{B}_d^{*}| = |B^{\bar{c}}|$ so, we necessarily have $\mathcal{A}_d^{*} \neq \mathcal{B}_d^{*}$.
	Second, in view of the fact that $d \sqsubseteq_{A,B} c$, although the two multisets may generally contain more than one colour, these colours cannot appear outside of these last ones. More formally, by construction we have that 
	$$
		\forall x \in A^{\bar{c}} \cup B^{\bar{c}}, y \in \tilde{A}^{\bar{c}} \cup \tilde{B}^{\bar{c}} \quad c_{x} \neq c_{y}
	$$
	\noindent and, due to $d \sqsubseteq_{A,B} c$ it must also hold that:
	$$
		\forall x \in A^{\bar{c}} \cup B^{\bar{c}}, y \in \tilde{A}^{\bar{c}} \cup \tilde{B}^{\bar{c}} \quad d_{x} \neq d_{y}
	$$
	This implies that, if we define multisets
	$$
		\tilde{\mathcal{A}_d^{*}} = \ldblbrace d_a | a \in \tilde{A}^{\bar{c}} \rdblbrace,
		\tilde{\mathcal{B}_d^{*}} = \ldblbrace d_b | b \in \tilde{B}^{\bar{c}} \rdblbrace
	$$
	\noindent then $(\mathcal{A}_d^{*} \cup \mathcal{B}_d^{*}) \cap (\tilde{\mathcal{A}_d^{*}} \cup \tilde{\mathcal{B}_d^{*}}) = \O$.

	Now, we have that $\mathcal{A}_d = \mathcal{A}_d^{*} \cup \tilde{\mathcal{A}_d^{*}}, \mathcal{B}_d = \mathcal{B}_d^{*} \cup \tilde{\mathcal{B}_d^{*}}, \mathcal{A}_d^{*} \neq \mathcal{B}_d^{*}$. Say that, w.l.o.g., this last holds due to a colour $\bar{d}$ appearing $n_A$ times in $\mathcal{A}_d^{*}$ and $n_B$ times in $\mathcal{B}_d^{*}$ with $n_A > n_B$. Then, a necessary condition for $\mathcal{A}_d = \mathcal{B}_d$ is that $\bar{d}$ appears $n_A - n_B$ times more in $\tilde{\mathcal{B}_d^{*}}$ than in $\tilde{\mathcal{A}_d^{*}}$. However, this condition cannot be met due to the disjointness of the multisets as shown above.
\end{proof}

\begin{proposition}\label{prop:multiset_equality_under_inj}
	Let $A$, $B$ be two multisets with elements in $\mathcal{D}$ such that $A = \ldblbrace a_i \rdblbrace_{i=1}^{m} = \ldblbrace b_i \rdblbrace_{i=1}^{m} = B$. For any injection $\varphi: \mathcal{D} \rightarrow \mathcal{C}$ it holds $\varphi(A) = \ldblbrace \varphi(a_i) \rdblbrace_{i=1}^{m} = \ldblbrace \varphi(b_i) \rdblbrace_{i=1}^{m} = \varphi(B)$.
\end{proposition}
\begin{proof}
	Let us suppose, for the sake of contradiction, that $\varphi(A) \neq \varphi(B)$. Thus, we can assume, w.l.o.g., that there exists an image $\bar{c}$ such that $\bar{c}$ appears more times in $\varphi(A)$ than in $\varphi(B)$, that is
	$$
		|\{ c_A | c_A = \bar{c}, c_A \in \varphi(A) \}| > |\{ c_B | c_B = \bar{c}, c_B \in \varphi(B) \}|
	$$
	If $\varphi$ is an injection, then $\forall c \in Im(\varphi) \subseteq \mathcal{C}$ there exists \emph{unique} $d \in \mathcal{D}$ such that $c = \varphi(d)$. This implies that there exist $d_A, d_B, \bar{d}$ such that we can rewrite the inequality above as:
	$$
		|\{ \varphi(d_A) | \varphi(d_A) = \varphi(\bar{d}), d_A \in A \}| > |\{ \varphi(d_B) | \varphi(d_A) = \varphi(\bar{d}), d_B \in B \}|
	$$
	\noindent and then
	$$
		|\{ d_A | d_A = \bar{d}, d_A \in A \}| > |\{ d_B | d_B = \bar{d}, d_B \in B \}|
	$$
	\noindent which would immediate entail $A \neq B$, against our hypothesis.
\end{proof}

\todo[inline]{FF: Probably this can be proved even more rigorously by leveraging on proposition \ref{prop:ref_implication} and \ref{prop:multiset_equality_under_inj} by defining a proper colouring which refines as we consider the entire tuples.}
\begin{proposition}\label{prop:tuple_multiset_equality_transfers_at_each_el}
	Let $A$, $B$ be two multisets with elements in $\mathcal{D}^1 \times \mathellipsis \times \mathcal{D}^k$ such that $A = \ldblbrace (a_i^1, \mathellipsis, a_i^k) \rdblbrace_{i=1}^{m}, \ldblbrace (b_i^1, \mathellipsis, b_i^k) \rdblbrace_{i=1}^{m} = B$. Let $A^j = \ldblbrace a_i^j \rdblbrace_{i=1}^{m}, B^j = \ldblbrace b_i^j \rdblbrace_{i=1}^{m}, \forall j = 1, \mathellipsis, k$. Then $A=B$ implies $A^j = B^j$.
\end{proposition}
\begin{proof}
	Let us suppose, for the sake of contradiction, that $A^j \neq B^j$. Thus, we can assume, w.l.o.g., that there exists $c$ such that $c$ appears more times in $A^j$ than in $B^j$. Let us define the set of indices
	$$
		I_{A^j_c} = \{ i^j | a_i^j \in A^j, a_i^j = c \}, I_{B^j_c} = \{ i^j | b_i^j \in B^j, b_i^j = c \}
	$$
    \noindent so that corresponding sets indexing the same elements in multisets $A, B$ are defined as:
	$$
		I_{A_c} = \{ i | a_i = (\cdot, \mathellipsis, a_i^j, \mathellipsis, \cdot) \in A, i^j \in I_{A^j_c} \}, I_{B_c} = \{ i | a_i = (\cdot, \mathellipsis, b_i^j, \mathellipsis, \cdot) \in B, i^j \in I_{B^j_c} \}
	$$
	\noindent with $|I_{A_c}| = |I_{A^j_c}| \neq |I_{B^j_c}| = |I_{B_c}|$.
	These sets induce a natural partitioning over $A, B$:
	$$
		A = A_c \cup \bar{A_c}, A_c = \ldblbrace a_i | i \in I_{A_c} \rdblbrace, \bar{A_c} = \ldblbrace a_i | i \notin I_{A_c} \rdblbrace
	$$
	\noindent and
	$$
	    B = B_c \cup \bar{B_c}, B_c = \ldblbrace a_i | i \in I_{B_c} \rdblbrace, \bar{B_c} = \ldblbrace b_i | i \notin I_{B_c} \rdblbrace
	$$
	Note that $A_c$ and $B_c$ represent the multisets of all and only those tuples having value $c$ as their $j$-th element.
	First, we observe that $A_c \neq B_c$, simply because the two have different cardinalities. Now, if $\bar{A_c} = \bar{B_c}$ we immediately have $A \neq B$, against our hypothesis. In fact, the contradiction arises also in the case $\bar{A_c} \neq \bar{B_c}$. Say, w.l.o.g. $A_c \neq B_c$ due to a tuple $d$ showing up $n_a$ times in the former multiset and $n_b$ times in the latter, with $n_a > n_b$. In this case, in order to have $A = B$ we must have that $d$ shows up exactly $n_a - n_b$ times more in $\bar{B_c}$ than in $\bar{A_c}$. However, $d \notin \bar{A_c} \cup \bar{B_c}$, because, by construction, no tuple with a $c$-valued $j$-th element belongs to either of the two multisets.
\end{proof}

\begin{definition}\label{def:vertex_set_preserving_policy}
	Let $G = (V, E)$ be any graph. Let $\rho$ be any subgraph selection policy generating an $m$-card deck $\mathcal{S}^{\rho}_G = \{ G_i = (V_i, E_i) \}_{i=1}^{m}$ over $G$. Policy $\rho$ is said to be \emph{vertex set preserving} if $\forall i = 1, \mathellipsis, m, V_i = V$.
\end{definition}

\begin{definition}\label{def:needle_node_colours}
	Let $G = (V, E)$ be a graph. Let $\rho$ be a \emph{vertex set preserving} policy generating an $m$-card deck $\mathcal{S}^{\rho}_G = \{ G_i \}_{i=1}^{m}$. The \emph{needle node colour} for node $v \in V$ at time step $t \in \mathbb{N}$, denoted $C_v^{(t)}$, is defined as $\ldblbrace c_{v,k}^{(t)} | k = 1, \mathellipsis, m \rdblbrace$, where $c_{v,k}^{(t)}$ is the node colour DSS-WL assigns to node $v$ on card $k$ at time step $t$. We remark that the \emph{needle node colour} $C_v^{(t)}$ is employed by such algorithm to obtain a refinement at time step $(t+1)$.
\end{definition}

\todo[inline]{FF: discuss the cardinality of the decks here}
\begin{lemma}\label{lem:dsswl_refines_wl}
	Let $\rho$ be any \emph{vertex set preserving} policy. Let $b^{\rho}$ denote the (needle) node colouring from DSS-WL running on decks induced by $\rho$, and $a$ be the node colouring from the standard WL algorithm. Then $b^{\rho} \sqsubseteq a$, that is, for all graphs $G^1 = (V^1, E^1)$ and $G^2 = (V^2, E^2)$ and all nodes $v \in \mathcal{V}^1, w \in \mathcal{V}^2$ we have that $b^{\rho}_v = b^{\rho}_w \implies a_v = a_w$.
\end{lemma}
\begin{proof}
	Let $G^1, G^2$ be any two graphs, $a^{(t)}$ refer to the WL colouring at iteration $t$, and $b^{(t)}$ refer to the needle colouring induced by DSS-WL at the same iteration (we drop the superscript $\rho$ to ease the notation). We seek to prove that $b^{(t)} \sqsubseteq a^{(t)} \forall t \geq 0$. We prove the lemma by induction on time step $t$.

	In particular, let us refer with $a^{(t)}_v$ to the WL-colour assigned to node $v$ at time step $t$, and with $b^{(t)}_v$ to the needle node colour DSS-WL assigns to the same node at the same iteration. We remark that this last is defined as $b^{(t)}_v = C^{(t)}_v = \ldblbrace c^{(t)}_{v,k} \rdblbrace_{k=1}^{m} $, with $c^{(t)}_{v,k}$ the DSS-WL colour assigned to node $v$ at time step $t$ on card $k$.

	\emph{(Base case)} At $t=0$, it clearly holds that $b^{(0)} \sqsubseteq a^{(0)}$ given that all nodes are initialised with the same constant colour $\bar{c}$.

	\emph{(Step)} Let us assume the thesis holds true at time step $t$: $b_{v}^{(t)} = b_{w}^{(t)} \implies a_{v}^{(t)} = a_{w}^{(t)}$. We seek to prove that if that is the case, it also holds true at time step $t+1$.

	Suppose $b_{v}^{(t+1)} = b_{w}^{(t+1)}$. Unrolling one step backwards in time we get:
	$$
		\ldblbrace \mathrm{g} (b_{v,k}^{(t)}, N_{v,k}^{(t)}, C_{v}^{(t)}, M_{v}^{(t)}) \rdblbrace_{k=1}^{m} = \ldblbrace \mathrm{g} (b_{w,k}^{(t)}, N_{w,k}^{(t)}, C_{w}^{(t)}, M_{w}^{(t)}) \rdblbrace_{k=1}^{m}
	$$
	\noindent where $g = \mathrm{HASH}$. In view of Proposition~\ref{prop:multiset_equality_under_inj}, the following equality also holds:
	$$
		\ldblbrace \mathrm{g}^{-1} \circ \mathrm{g} (b_{v,k}^{(t)}, N_{v,k}^{(t)}, C_{v}^{(t)}, M_{v}^{(t)}) \rdblbrace_{k=1}^{m} = \ldblbrace \mathrm{g}^{-1} \circ \mathrm{g} (b_{w,k}^{(t)}, N_{w,k}^{(t)}, C_{w}^{(t)}, M_{w}^{(t)}) \rdblbrace_{k=1}^{m}
	$$
	\noindent since, due to the injectivity of $g$, the left inverse $\mathrm{g}^{-1}: Im(g) \rightarrow D(g)$ exists and is injective. Thus we have:
	$$
		\ldblbrace (b_{v,k}^{(t)}, N_{v,k}^{(t)}, C_{v}^{(t)}, M_{v}^{(t)}) \rdblbrace_{k=1}^{m} = \ldblbrace (b_{w,k}^{(t)}, N_{w,k}^{(t)}, C_{w}^{(t)}, M_{w}^{(t)}) \rdblbrace_{k=1}^{m}
	$$
	\noindent where, in view of Proposition~\ref{prop:tuple_multiset_equality_transfers_at_each_el}, we also have:
	$$
		\ldblbrace (C_{v}^{(t)}) \rdblbrace_{k=1}^{m} = \ldblbrace (C_{w}^{(t)}) \rdblbrace_{k=1}^{m}, \quad
		\ldblbrace (M_{v}^{(t)}) \rdblbrace_{k=1}^{m} = \ldblbrace (M_{w}^{(t)}) \rdblbrace_{k=1}^{m}
	$$
	The elements of these multisets do not depend on index $k$, therefore we can rewrite the equalities as the set equalities:
	$$
		\{ (C_{v}^{(t)}, m) \} = \{ (C_{w}^{(t)}, m) \}, \quad
		\{ (M_{v}^{(t)}, m) \} = \{ (M_{w}^{(t)}, m) \}
	$$
	\noindent which obviously imply
	$$
		C_{v}^{(t)} = C_{w}^{(t)}, \quad
		M_{v}^{(t)} = M_{w}^{(t)}
	$$

	First, we note that $b_{v}^{(t)} = C_{v}^{(t)} = C_{w}^{(t)} = b_{w}^{(t)}$, which by the induction hypothesis gives us $a_{v}^{(t)} = a_{w}^{(t)}$.

	Second, we note that $M_{v}^{(t)} = \ldblbrace b_{i}^{(t)} | i \in \mathcal{N}(v) \rdblbrace$ and $M_{w}^{(t)} = \ldblbrace b_{j}^{(t)} | j \in \mathcal{N}(w) \rdblbrace$. By the induction hypothesis we then have $\ldblbrace a_{i}^{(t)} | i \in \mathcal{N}(v) \rdblbrace = \ldblbrace a_{j}^{(t)} | j \in \mathcal{N}(w) \rdblbrace$. This, along with the result above, implies $a_{v}^{(t+1)} = a_{w}^{(t+1)}$, since both the two inputs to hash $g$ at time step $t$ coincide. The proof terminates.
\end{proof}

\todo[inline]{FF: Probably this can be proved even more rigorously by leveraging on proposition \ref{prop:ref_implication} (I am thinking of the step about the transitive refinement).}
\begin{theorem}\label{thm:dsswl_at_least_as_powerful_as_wl}
	Let $\rho$ be any \emph{vertex set preserving} policy. DSS-WL on $\rho$-induced decks is at least as powerful as WL in distinguishing non-isomorphic graphs, i.e., any two non-isomorphic graphs $G^1, G^2$ distinguished by WL are also distinguished by DSS-WL when run on the respective $\rho$-induced decks.
\end{theorem}
\begin{proof}
	Throughout the proof, we will denote with $a$ colourings generated by the WL algorithm, while $b$ will generally denote colourings generated by DSS-WL. Additionally, we denote as $\mathcal{D}^1, \mathcal{D}^2$ the $\rho$-decks of, respectively, $G^1, G^2$. We suppose the two decks have both cardinality $m$, and are defined as $\mathcal{D}^1 = \ldblbrace G^1_k = (V^1, E^1_k) \rdblbrace_{k=1}^{m}, \mathcal{D}^2 = \ldblbrace G^2_h = (V^2, E^2_h) \rdblbrace_{h=1}^{m} $. We do not explicitly focus on the case $|\mathcal{D}^1| \neq |\mathcal{D}^2|$ as the two graphs would then be (trivially) distinguished by DSS-WL.

	Let us start by recalling that at time step $t$, two graphs are deemed non-isomorphic by the WL algorithm when the two are assigned two distinct multisets of \emph{node colours}:
	$$
		\ldblbrace a_v^{(t)} | v \in V^1 \rdblbrace \neq \ldblbrace a_w^{(t)} | w \in V^2 \rdblbrace
	$$
	\noindent while the DSS-WL algorithm deems them non-isomorphic when the two are assigned two distinct multisets of \emph{card colours}, that is:
	$$
		\ldblbrace b_{G^1_k}^{(t)} \rdblbrace_{k=1}^{m} \neq \ldblbrace b_{G^2_h}^{(t)} \rdblbrace_{h=1}^{m}
	$$
	\noindent where $b_{G^i_j}^{(t)}$ generally indicates the colour computed for card $j$ of graph $G^i$: $\ldblbrace b_{v,j}^{(t)} | v \in V^i \rdblbrace$.

	Suppose WL distinguishes between the two graphs at iteration $T$. In view of Lemma~\ref{lem:dsswl_refines_wl}, we know that $b^{(T)} \sqsubseteq a^{(T)}$, where $b^{(T)}$ is the needle node colouring generated by DSS-WL at time step $T$. At the same time, it can be shown that $b^{(T)}$ is refined by the colouring generated by DSS-WL at the following time-step on any pair of cards. That is:
	$$
	b_{v,k}^{(T+1)} = b_{w,h}^{(T+1)} \implies b_{v}^{(T)} = b_{w}^{(T)} \quad \forall h, k \in \{1, \mathellipsis, m\} \quad \forall v \in V^1, w \in V^2 
	$$
	The antecedent implies the equality of all inputs to the $\mathrm{HASH}$ function at time step $T$, that is: $b_{v,k}^{(T)} = b_{w,h}^{(T)}, N_{v,k}^{(T)} = N_{w,h}^{(T)}, M_{v}^{(T)} = M_{w}^{(T)}$ and, importantly, $C_{v}^{(T)} = C_{w}^{(T)}$. By the definition of needle node colours, this last equality is rewritten as $b_{v}^{(T)} = b_{w}^{(T)}$, which proves the refinement.

	This tells us that, by transitivity, if two graphs are deemed non-isomorphic by the WL algorithm at step $T$, then at step $T+1$, DSS-WL assigns a distinct colour to any pair of cards from the respective decks, that is:
	$$
		b_{G^1_k}^{(T+1)} = \ldblbrace b_{v,k}^{(T+1)} | v \in V^1 \rdblbrace \neq \ldblbrace b_{w,h}^{(T+1)} | w \in V^2 \rdblbrace = b_{G^2_h}^{(T+1)}, \forall h, k \in \{1, \mathellipsis, m\}
	$$
	
	This immediately leads DSS-WL to distinguish between graphs $G^1, G^2$ as their corresponding multisets of card colours are disjoint.
\end{proof}

\begin{lemma}\label{lem:dsswl_noderefines_wl}
	Let $\rho$ be any subgraph selection policy, $G^1, G^2$ be any two graphs and $\mathcal{D}^1, \mathcal{D}^2$ the $\rho$-decks thereof, with $\mathcal{D}^1 = \ldblbrace G^1_k = (V^1_k, E^1_k) \rdblbrace_{k=1}^{m^{(1)}}, \mathcal{D}^2 = \ldblbrace G^2_h = (V^2_h, E^2_h) \rdblbrace_{h=1}^{m^{(2)}}$.
	Let $a^{G, (t)}$ refer to the colouring generated by $t$ steps of the WL algorithm run over graph $G \in \mathcal{D}_1 \cup \mathcal{D}_2$ and let $b^{G, (t)}$ refer to the colouring generated by DSS-WL on the same graph.
	Then, for any $t \geq 0$, $\forall G = (V_G, E_G), F = (V_F, E_F) \in \mathcal{D}_1 \cup \mathcal{D}_2, \forall v \in V_G, w \in V_F, b^{G, (t)}_v = b^{F, (t)}_w \implies a^{G, (t)}_v = a^{F, (t)}_w$.
\end{lemma}
\begin{proof}
	As usual, let us prove the lemma by induction on $t$.

	The thesis trivially holds for $t=0$ given that all nodes in all cards are assigned the same colour. Let us assume the thesis holds true for $t>0$, we seek to show it also holds for $t+1$.

	Suppose $b^{G, (t+1)}_v = b^{F, (t+1)}_w$. The equality can be rewritten as $\mathrm{HASH}(b^{G, (t)}_v, N^{G, (t)}_v, C^{(t)}_v, M^{(t)}_v) = \mathrm{HASH}(b^{F, (t)}_w, N^{F, (t)}_w, C^{(t)}_w, M^{(t)}_w)$, which implies the equality between each of the inputs to the $\mathrm{HASH}$ function. Importantly, this means that $b^{G, (t)}_v = b^{F, (t)}_w$ and $N^{G, (t)}_v = N^{F, (t)}_w$. The induction hypothesis immediately gives us $a^{G, (t)}_v = a^{F, (t)}_w$ and $\ldblbrace a^{G, (t)}_i | i \in \mathcal{N}^G(v) \rdblbrace = \ldblbrace a^{F, (t)}_j | j \in \mathcal{N}^F(w) \rdblbrace$, by the definition of $N^{G, (t)}_v$ and $N^{F, (t)}_w$. These are equalities between the (only) inputs in the WL colour refinement step, which applies an injective $\mathrm{HASH}$ to obtain $a^{G, (t+1)}_v$ and $a^{F, (t+1)}_w$. It then immediately follows that $a^{G, (t+1)}_v = a^{F, (t+1)}_w$.
\end{proof}

\todo[inline]{FF: Probably this can be proved even more rigorously by leveraging on proposition \ref{prop:ref_implication} and \ref{prop:multiset_equality_under_inj} and this would turn it into the more general relation between refinement at the level of nodes and refinement at the level of cards}
\begin{corollary}\label{cor:dsswl_cardrefines_dswl}
	Let $\rho$ be any subgraph selection policy, $G^1, G^2$ be any two graphs and $\mathcal{D}^1, \mathcal{D}^2$ the $\rho$-decks thereof, with $\mathcal{D}^1 = \ldblbrace G^1_k = (V^1_k, E^1_k) \rdblbrace_{k=1}^{m^{(1)}}, \mathcal{D}^2 = \ldblbrace G^2_h = (V^2_h, E^2_h) \rdblbrace_{h=1}^{m^{(2)}}$. Let $a^{(t)}_G$ and $b^{(t)}_G$ refer to the card colours assigned to card $G$ at step $t$ by, respectively, DS-WL and DSS-WL.
	For any pair of cards $G, F \in \mathcal{D}_1 \cup \mathcal{D}_2$, and time step $t \in \mathbb{N}$, if DS-WL assigns a distinct colour to $G$ and $F$ then DSS-WL does so as well: $a^{(t)}_G \neq a^{(t)}_F \implies b^{(t)}_G \neq b^{(t)}_F$.
\end{corollary}
\begin{proof}
	In both algorithms, card colours are obtained by injectively hashing the multisets of node colours therein. Furthermore, in DS-WL, the node colours at time step $t$ on generic card $G$ are obtained by independently running $t$ rounds of the WL procedure on $G$. This implies that if two cards are assigned different colours by DS-WL at time step $t$, then the underlying graphs are deemed non-isomorphic by the WL algorithm at time step $t$. In view of Lemma~\ref{lem:dsswl_noderefines_wl}, then the same cards must therefore be assigned different colours by DSS-WL at the same time step. This must be the case, otherwise we would have two (sub)graphs distinguished by the WL colouring at $t$, which cannot be distinguished by the DSS-WL colouring at the same step, in contrast with the above Lemma~\ref{lem:dsswl_noderefines_wl} stating instead that the latter refines the former.
\end{proof}

\todo[inline]{FF: Do we need to say sth about the policy?}
\begin{proposition}\label{prop:dsswl_at_least_as_powerful_as_dswl}
	Let $\rho$ be any subgraph selection policy. When both are run on the same $\rho$-induced decks, DSS-WL is at least as powerful as DS-WL in distinguishing non-isomorphic graphs, i.e., any two non-isomorphic graphs $G^1, G^2$ distinguished by DS-WL via policy $\rho$ are also distinguished by DSS-WL via the same policy.
\end{proposition}
\begin{proof}
	Let $\mathcal{D}^1 = \ldblbrace G^1_k \rdblbrace_{k=1}^{m}, \mathcal{D}^2 = \ldblbrace G^2_h \rdblbrace_{h=1}^{m}$ be the decks induced by $\rho$ on $G_1, G_2$. Let $a^{(t)}$ and $b^{(t)}$ refer to the card colouring computed at step $t$ by, respectively, DS-WL and DSS-WL.
	The theorem immediately follows in light of Corollary~\ref{cor:dsswl_cardrefines_dswl} and Proposition~\ref{prop:ref_implication}. Let $\mathcal{D}^1, \mathcal{D}^2$ correspond to, respectively sets $A, B$ from Proposition~\ref{prop:ref_implication}, and let $a^{(T)}, b^{(T)}$ correspond to, respectively, colourings $c, d$ from the same proposition. If $G^1, G^2$ are distinguished by DS-WL at step $T$, then we have $\mathcal{A}_c \neq \mathcal{B}_c$. Also, in view of Corollary~\ref{cor:dsswl_cardrefines_dswl}, it holds that $b^{(T)} \sqsubseteq_{\mathcal{D}^1, \mathcal{D}^2} a^{(T)}$, that is $d \sqsubseteq_{A,B} c$. All hypotheses in Proposition~\ref{prop:ref_implication} hold and we can then conclude that $\mathcal{A}_d \neq \mathcal{B}_d$ that is $\mathcal{A}_{b^{(T)}} \neq \mathcal{B}_{b^{(T)}}$. This shows DSS-WL assigns the two decks distinct multisets of colours, and thus, as DS-WL, it distinguishes between the two graphs $G^1, G^2$.
\end{proof}

\begin{lemma}\label{lem:cardwl_refines_wl}
    Let $\rho$ be any subgraph selection policy such that $\forall G, \mathcal{S}_{G}^\rho = \mathcal{S}_{G}^\rho \cup \{ G \}$, with $\mathcal{S}_{G}^\rho$ denoting the deck induced by $\rho$ on $G$. DS-WL on $\rho$-induced decks is at least as powerful as WL in distinguishing non-isomorphic graphs, i.e., any two non-isomorphic graphs $G^1, G^2$ distinguished by WL are also distinguished by DS-WL when run on the respective $\rho$-induced decks.
\end{lemma}
\begin{proof}
    Let $G^1, G^2$ be two graphs distinguished by WL. We focus on the non-trivial case in which the two graphs have the same number of edges (and nodes) and policy $\rho$, on the two graphs, generates decks of same cardinality. Let $T \geq 1$ be the round at which the WL procedure has converged on each card. Let us denote by $a^1, a^2, a^1 \neq a^2$ the representations WL assigns to the two graphs at time step $T$ and by $C^1 = \ldblbrace c^{1}_k \rdblbrace_{k=0}^{m}, C^2 = \ldblbrace c^{2}_k \rdblbrace_{k=0}^{m}$ the multisets of \emph{card} colours computed by DS-WL on the two input $\rho$-decks at the same step. In particular, let $c^{1}_0, c^{2}_0$ be the card colours associated with the (sub)graphs $G_\top^1 = G^1, G_\top^2 = G^2$. Clearly, $c^{1}_0 = a^{1}, c^{2}_0 = a^{2}, c^{1}_0 \neq c^{2}_0$ since they are obtained by running an independent WL procedure on $G_\top^1 = G^1, G_\top^2 = G^2$ for the same number of steps.
    
    We note that $ \forall k=1, \mathellipsis, m, i=1,2, c^{i}_k \notin \{ c^{1}_0, c^{2}_0 \}$. This is because, any other card from any deck has a number of edges smaller than the one in the original graphs and it is known that WL can count the number of edges with $1$ refinement round~\todo[inline]{FF: It would be good to find a reference for this}. This immediately implies the presence of a colour in $C^1$ which is not in $C^2$ (and vice-versa), thus $C^1 \neq  C^2$ which entails DS-WL distinguishes between the two graphs.
\end{proof}

\begin{theorem}\label{th:cardwl_vs_wl}
    Let $\rho$ be either the node- or edge-deletion policy and $\mathcal{S}_{G}^\rho$ represent the subgraph collection induced by $\rho$ on graph $G$, for any $G$. DS-WL on deck $\mathcal{S}_{G}^\rho \cup \{ G \}$ is strictly more powerful than WL in distinguishing between non-isomorphic graphs.
\end{theorem}
\begin{proof}
    Given Lemma~\ref{lem:cardwl_refines_wl}, it is sufficient to exhibit an exemplary pair of graphs that cannot be distinguished by WL but can be distinguished by Card-WL. One such pair is $(G_1, G_2)$, where $G_1$ is the chordless cycle graph with $6$ nodes and $G_2$ is the graph constituted by two disconnected triangles. The standard WL test converges at initialisation, whereas it can be easily verified that Card-WL outputs a different colour histogram for the two graphs already at iteration $t=2$.
\end{proof} 

We will now focus on characterising the relation between the proposed \texttt{WL} variants and neural counterparts such as the DSS-GNN architecture introduced above. 

















    
    
    
    
    
    
    
    
    
    
    
    
    





	

	






Before proving the theorem we first show that there exists a DSS-GNN architecture that can ``simulate'' the colour refinement steps of the DSS-WL algorithm.

\begin{lemma}\label{lem:dssgnn_simulates_dsswl}
    Let $\mathcal{G} = \{ G_i = (V_i, E_i) \}_{i=1}^{m}$ denote the deck generated by a subgraph selection policy applied on any graph $G = (V, E)$ such that $\forall e \in E, e \in \cup_{i=1}^{m} E_i$. Let $c_{v,k}^{(T)}$ be the colour assigned by DSS-WL to node $v$ in card $k$, after $T$ iterations. There exists a DSS-GNN model $\mathcal{M}$ with $D = 10T$ layers of the form described in Equation~\ref{eq:linear_dssgnn} such that $c_{v,k}^{(T)}$ is uniquely represented by a one-hot encoding $h_{v,k}^{(D)}$, the representation for node $v$ in card $k$ computed by such a model.
\end{lemma}

\begin{proof}

	We will prove the lemma by describing how to parameterise the DSS-GNN layers in a way to simulate the DSS-WL colour refinement step on each card.

	\emph{(Preliminaries)} In this proof we assume to work with finite graphs whose degree is upper-bounded by a positive integer $N \in \mathbb{N}$. From these assumptions it immediately follows that any employed subgraph selection policy generates a finite deck whose cards are finite subgraphs with degree upper-bounded by $N$. For a DSS-GNN to simulate colour refinement steps, it is necessary to encode colours in vector/matrix form. As we are working with finite graphs (of bounded degree), at any step, each of the four inputs in the DSS-WL colour refinement equation belongs to a finite set. The domain of the $\mathrm{HASH}$ function is therefore  represented by the cross-product of such these finite sets and is therefore finite. $\mathrm{HASH}$ is an injective function with finite domain; its image must therefore be finite. The application of this injective function effectively computes a unique representation of the inputs by assigning them a colour. 

	\emph{(Encoding)} Given these premises, it is clear that, at each time step, it is possible to represent colours as one-hot vectors of proper dimension without losing any information. This allows the application of our DSS-GNN model. In the following, we indicate with $t \in \mathbb{N}$ a time step in the DSS-WL procedure, and with $d_t \in \mathbb{N}$ the corresponding layer of the described DSS-WL model. Note that, in general, $d_t \geq t$ as more than one layer is required to simulate one colour refinement step. Let $c_{v,k}^{(t)}$ be the colour assigned to node $v$ on card $k$ at time-step $t$ and $h_{v,k}^{(d_t)}$ be its representation computed by our DSS-GNN model, of dimension $a_{d_t}$. At time step $t=0$, each node in each card is assigned a constant colour $c_{v,k}^{(0)} = \bar{c}$; if initial colours are available, they are retained. We consider $h_{v,k}^{(d_0)} = h_{v,k}^{(0)}$ to be a proper one-hot encoding of these initial colours. For a colour refinement from time step $t$ to $t+1$ we consider inputs to layer $d_t$ to be one-hot encoded. The refinement is simulated with layers $d_t$ to $d_{t+1}$, where the final output of these is a one-hot encoding uniquely representing the result of the $\mathrm{HASH}$ function.

	\emph{(Computation)} Starting from the one-hot colour representation in input to layer $d_t$, the refinement step is implemented by: (i) computing unique representations for all the four inputs to the $\mathrm{HASH}$ function; (ii) simulating the $\mathrm{HASH}$ function by mapping them to an output, unique, one-hot encoding.
	Let us start by describing step (i). An important observation is that the summation is an injective aggregator over multisets when elements are represented by one-hot encodings. In other words, we can uniquely represent a multiset of one-hot encoded elements by simply summing its members. This implies that there exists one DSS-GNN layer which computes a unique representation for each of the first three inputs to the $\mathrm{HASH}$ function: $c_{v,k}^{(t)}, N_{v,k}^{(t)}, C_{v}^{(t)}$. In this layer, each matrix $ W $ has dimension $ 3 \cdot a_{d_t} \times a_{d_t}$ and $ b $ has dimension $ 3 \cdot a_{d_t} $. In particular: $ W^1_1 = [ I, \mathbf{0}, \mathbf{0} ], W^1_2 = [ \mathbf{0}, I, \mathbf{0} ], W^2_1 = [ \mathbf{0}, \mathbf{0}, I ], W^2_2 = \mathbf{0}, b = \mathbf{0} $, where $[\cdot , \cdot]$ indicates vertical concatenation.
	
	In output from this layer are vectors in the form $ h_{v,k}^{(d_t + 1)} = [h_{v,k}^{(d_t)}, h_{v,k}^{(d_t, N)}, h_{v}^{(d_t, C)}] $, with the last two components representing unique encodings of, respectively, inputs $N_{v,k}^{(t)}, C_{v}^{(t)}$.
	In order to also compute a unique representation for the fourth input ($M_{v}^{(t)}$), we cannot directly apply summation on the just computed $h_{v}^{(d_t, C)}$, because these are not one-hot encoded anymore, and summation is, generally, not injective. To overcome this, we employ additional layers to first uniquely encode each $h_{v,k}^{(d_t, C)}$ with a one-hot scheme so that the original neighborhoods $\mathcal{N}(v)$ would be uniquely encoded by the summation over them, inherent in the DSS-GNN layer. This one-hot encoding scheme is possible because there is only a finite number of multisets of cardinality $m$ that can be constructed from a finite colour palette of cardinality $a_{d_t}$. Additionally, this encoding can be computed by stacking $4$ DSS-GNN layers with ReLU activations as shown by the following:

	\begin{lemma}\label{lem:dssgnn_onehotencodes_elements_from_finite_set}
		Let $\mathcal{H}$ be a finite set. Let elements in $\mathcal{H}$ be uniquely encoded by $h(\cdot)$. There exists a $4$-layer DSS-GNN model which computes the map $\mu: h(a) \mapsto e, a \in \mathcal{H}$ with $e$ being a unique one-hot encoding for element $a$.
	\end{lemma}
	\begin{proof}
		We consider an ordering relation $ < $ determining an overall sorting $s$ of the multisets in $\mathcal{H}$. This can be obtained, for example, by a lexicographic ordering of the elements in the encodings $h(\cdot)$. This sorting associates any element with an integer index, that is $s: \mathcal{H} \rightarrow \mathbb{N}, s: a \mapsto i$. We can therefore denote each (encoded) element with $h_i, i = 1, \mathellipsis, |\mathcal{H}|$. We seek to implement the mapping $\mu: h_i \mapsto e_i$, such that: $ e_i \in \{ 0, 1 \}^{|\mathcal{H}|} $ and $(e_i)_j = 1$ if $j = i$, $(e_i)_j = 0$ otherwise.
		
		We define the dataset $\mathcal{D} = \{ (h_i, e_i) \}_{i=1}^{\mathcal{H}}$. This dataset satisfies Assumption $3.1$ in~\citet{yun2019small}: all $h_i$'s are distinct and labels $e_i$'s are in $[-1, +1]^{d_y}, d_y = |\mathcal{H}|$. Moreover we have that $\forall i, e_i \in {0, 1}^{d_y}$. Thus, according to Proposition 3.2 in the same work, there exists a $4$-layer ReLU network parameterised by $\mathbf{\theta}$ and with $\Omega(\sqrt{|\mathcal{H}|} + |\mathcal{H}|)$ neurons which perfectly fits $\mathcal{D}$. This network computes $\mu$ and is exactly implemented by a $4$-layer DSS-GNN model with matrices ${W^1_2}^{(l)}, {W^2_1}^{(l)}, {W^2_2}^{(l)} = \mathbf{0}, l=1, \mathellipsis, 4$ and $\mathbf{\theta} = {({W^1_1}^{(l)}, b^{(l)})}_{l=1}^4$.
	\end{proof}

	In view of Lemma~\ref{lem:dssgnn_onehotencodes_elements_from_finite_set}, there exists a stacking of $4$ DSS-GNN layers such that $ h_{v,k}^{(d_t + 5)} = [h_{v,k}^{(d_t)}, h_{v,k}^{(d_t, N)}, \bar{h}_{v}^{(d_t, C)}] $, with $\bar{h}_{v}^{(d_t, C)}$ being the one hot encoding of $h_{v}^{(d_t, C)}$, dimension $e_{t, C}$.
	If ${(\tilde{W^1_1}^{(l)}, \tilde{b}^{(l)})}_{l=d+1}^{d+5}$ are the parameters from Lemma~\ref{lem:dssgnn_onehotencodes_elements_from_finite_set} one-hot encoding $h_{v}^{(d_t, C)}$, then these layers are obtained simply by ${W^1_1}^{(l)} = [ [ I | \mathbf{0} ] , [ \mathbf{0} | \tilde{W^1_1}^{(l)} ] ], b^{l} = [\mathbf{0}, \tilde{b}^{(l)}], {W^1_2}^{(l)}, {W^2_1}^{(l)}, {W^2_2}^{(l)} = \mathbf{0}$. Here $[ \cdot | \cdot ]$ indicates horizontal concatenation and $I$ is always of size $2 \cdot a_{d_t} \times 2 \cdot a_{d_t}$.
	Overall, each $h_{v,k}^{(d_t + 5)}$ has dimension $a_{d_t+5} = (2 \cdot a_{d_t}) + e_{t, C}$. Importantly, we notice that component $\bar{h}_{v}^{(d_t, C)}$ is computed for node $v$ but independently of $k$, and is thus shared across all cards.
	Layer $d_t + 6$ now computes the encoding of $M_{v}^{(t)}$. Each weight matrix has dimension $( a_{d_t+5} + e_{t, C} ) \times a_{d_t+5}$ with: $ W^1_1 = [ I, \mathbf{0} ]$ ($I$ size $a_{d_t+5}$), $W^1_2, W^2_1 = \mathbf{0}, W^2_2 = [ \mathbf{0}, [ \mathbf{0}_\bot | \frac{1}{m} I ] ]$ ( $\mathbf{0}_\bot$ size $ e_{t, C} \times (2 \cdot a_{d_t}) $, $I$ size $e_{t, C}$), $ b = \mathbf{0} \in \mathbb{R}^{a_{d_t+5}} $.

	Now, $h_{v,k}^{(d_t + 6)} = [h_{v,k}^{(d_t)}, h_{v,k}^{(d_t, N)}, \bar{h}_{v}^{(d_t, C)}, \bar{h}_{v}^{(d_t, M)}]$, of dimension $a_{d_t+6} = a_{d_t+5} + e_{t, C}$, constructed as the concatenation of unique representations of the inputs to the $\mathrm{HASH}$ function. It is only left to `simulate' the application of this last. We do this by computing a one-hot encoding of vector $h_{v,k}^{(d_t + 6)}$. As already discussed, this encoding is possible due the fact that $\mathrm{HASH}$ is an injection with domain of finite cardinality. In other words, vectors $h_{v,k}^{(d_t + 6)}$ can only assume a finite number of distinct values. Again, this encoding is computable by $4$ DSS-GNN layers, as per Lemma~\ref{lem:dssgnn_onehotencodes_elements_from_finite_set}.
	
	Finally, we have that $h_{v,k}^{(d_{t+1})} = h_{v,k}^{(d_t + 10)}$. This construction can be arbitrarily repeated to exactly simulate $T$ iterations of the DSS-WL colour refinement step with $D = 10T$ layers, which concludes the proof.

\end{proof}

\begin{lemma}\label{lem:dsgnn_simulates_dswl}
    Let $\mathcal{G} = \{ G_i \}_{i=1}^{m}$ denote the deck generated by a subgraph selection policy applied on any graph $G$. Let $c_{v,k}^{(T)}$ be the colour assigned by DS-WL to node $v$ in card $k$, after $T$ iterations. There exists a DS-GNN model $\mathcal{M}$ with $D = 5T$ layers of the form described in Equation~\ref{eq:linear_dssgnn} such that $c_{v,k}^{(T)}$ is uniquely represented by a one-hot encoding $h_{v,k}^{(D)}$, the representation for node $v$ in card $k$ computed by such a model.
\end{lemma}
\begin{proof}
    The proof closely follows the one for Lemma~\ref{lem:dssgnn_simulates_dsswl}; we work in the same regime (finite graphs of bounded degree) and assume the network encodes node colours with a proper one-hot encoding at each refinement step being simulated. The difference is that, in this case, the described DS-GNN model always has parameters $W^2_1, W^2_2 = \mathbf{0}$ and does not need to encode the $\mathrm{HASH}$ inputs $C_{v}^{(t)}, M_{v}^{(t)}$ (not present in the WL update equations).
    
    Let $c_{v,k}^{(t)}$ be the colour assigned to node $v$ on card $k$ at time-step $t$ and $h_{v,k}^{(d_t)}$ be its representation computed by our DS-GNN model, of dimension $a_{d_t}$ and properly one-hot encoded. We seek to describe a stacking of DS-GNN layers producing $h_{v,k}^{(d_{t+1})}$, a unique, one-hot encoding of colour $c_{v,k}^{(t+1)}$.
    
    Once more, since summation is an injective aggregator over multisets when elements are represented by one-hot encodings, there exists one DS-GNN layer which computes a unique representation for the two inputs to the $\mathrm{HASH}$ function: $c_{v,k}^{(t)}, N_{v,k}^{(t)}$. In this layer, each matrix $ W $ has dimension $ 2 \cdot a_{d_t} \times a_{d_t}$ and $ b $ has dimension $ 2 \cdot a_{d_t} $. In particular: $ W^1_1 = [ I, \mathbf{0} ], W^1_2 = [ \mathbf{0}, I ], b = \mathbf{0}$ where $[\cdot , \cdot]$ indicates vertical concatenation. 
	
	In output from this layer are vectors in the form $ h_{v,k}^{(d_t + 1)} = [h_{v,k}^{(d_t)}, h_{v,k}^{(d_t, N)}] $, with the last component representing a unique encoding of $N_{v,k}^{(t)}$. In order to obtain $ h_{v,k}^{(d_{t + 1})} $ it is only left to one-hot encode $ h_{v,k}^{(d_t + 1)} $. By Lemma~\ref{lem:dssgnn_onehotencodes_elements_from_finite_set}, this operation can be performed by a $4$-layer DSS-GNN which only leverages on matrix $W^1_1$ (in module $L_1$) and bias $b$, which is also a DS-GNN.
\end{proof}

\begin{theorem}
	For any two graphs $G^1, G^2$ distinguished by DSS-WL (resp. DS-WL) under subgraph selection policy $\rho$, there exists a DSS-GNN (resp. DS-GNN) architecture in the form of Equation~\ref{eq:dss-gnn-arch} with a sufficient number of layers of a sufficient width which, when equipped with the same selection policy, assigns $G^1, G^2$ distinct representations (and thus distinguishes them). In the case of DSS-WL, it is required that the selection policy is such that each edge in the original graph is present in at least one card.
\end{theorem}
\begin{proof}
	In this proof we will directly describe a DSS-GNN architecture satisfying the requirements. According to Equation~\ref{eq:dss-gnn-arch}, a DSS-GNN architecture computes a representation for a graph in input as: $h_G = E_{\text{sets}}\circ R_{\text{subgraphs}} \circ E_{\text{subgraphs}} (G)$. Let $T$ be the time step at which DSS-WL (resp. DS-WL) distinguishes two input graphs $G^1, G^2$. At this round, the overall colouring is such that the multisets of card colours for the two graphs are distinct:
	$$
		\ldblbrace c_{G^1_k}^{(T)} \rdblbrace_{k=1}^{m} \neq \ldblbrace c_{G^2_h}^{(T)} \rdblbrace_{h=1}^{m}
	$$
	\noindent where $c_{G^i_j}^{(T)}$ generally indicates the colour computed for card $j$ of graph $G^i$: $\mathrm{HASH}(\ldblbrace c_{v,j}^{(T)} | v \in V^i \rdblbrace)$.
	
	Now, let $E_{\text{subgraphs}}$ be the module obtained by the stacking described in Lemma~\ref{lem:dssgnn_simulates_dsswl} (resp. Lemma~\ref{lem:dsgnn_simulates_dswl}). We know that this module uniquely encodes each card node colour $c_{v,j}^{(T)}$ with one-hot representations $h_{v,j}^{(d_T)}$. Therefore, it is only left to describe modules $R_{\text{subgraphs}}, E_{\text{sets}}$ in a way to injectively aggregate such representations into an overall graph embedding.
	
	Given that card node colours are (uniquely) represented by one-hot encodings, the required $R_{\text{subgraphs}}$ can be simply obtained by summation over node representations on each card. This is because summation is an injective aggregator when multiset elements are described in a one-hot fashion. Let us generally refer to the computed card representations as $h_{j}$.
	
	Let us finally describe module $E_{\text{sets}}$. If the graphs of interest have a number of nodes upper-bounded by constant $M$, then $h_{j}$'s uniquely represent multisets of bounded size from a finite colour palette. They are finite in number, so it would be possible to compute a one-hot encoding for these card representations with a $4$-layer ReLU MLP applied in a siamese fashion. Lemma~\ref{lem:dssgnn_onehotencodes_elements_from_finite_set} ensures the existence of such a network as the described stacking of DSS-GNN layers effectively boils down to an MLP. This would constitute the first $4$ layers of $E_{\text{sets}}$. To conclude, one last layer applying summation to these one-hot encodings would suffice to output an embedding uniquely describing the multiset of card colours.
	
	If the size of input graphs is not upper-bounded by a constant, $E_{\text{sets}}$ can be constructed by resorting to a more general DeepSets model~\citep{zaheer2017deep} endowed with sum pooling and learnable universal approximators (such as MLPs). The card colours obtained by module $R_{\text{subgraphs}}$ are from a countable universe, and, under this condition, these models are universal multiset function approximators. This guarantees the existence of a $E_{\text{sets}}$ computing the desired injective mapping -- up to arbitrary precision -- and allows us to conclude the proof. 
\end{proof}




\section{WL formalisation}

We propose to approach the graph isomorphism testing problem from a different angle. Contrary to the standard WL algorithm, which refines colours at the level of nodes or edges, we instead consider colourings at the more general level of subgraphs. Given an input graph $G$ we apply a selection policy $\pi$ to obtain a (multi)set $\mathcal{S}^G_\pi$ of subgraphs. In resemblance with the reconstruction conjecture, we conveniently refer to $\mathcal{D} = \mathcal{S}^G_\pi$ as a \emph{deck} and to the included subgraphs as \emph{cards}. The idea is to test the isomorphism between graphs based on a representation of its associated deck.

Similarly to the WL algorithm, we can define the concept of \emph{deck colouring}:
\begin{definition}
    A deck colouring is a map $c$ that maps a deck $\mathcal{D}$ and one of its card $\mathcal{K}$ to a colour $c^\mathcal{D}_\mathcal{K}$ from a fixed palette. 
\end{definition}
When the deck is clear from the context, we use the lighter notation $c_\mathcal{K}$.

Given a deck colouring, we can employ it to represent the initial graph from which the subgraphs have been selected. We represent graph $G$ as the multiset of the associated card colours: $c_G = \ldblbrace c_\mathcal{K} | \mathcal{K} \in \mathcal{D} \rdblbrace$ (or an injection thereof). 

Similarly in spirit with other graph colouring algorithms, these card-based graph representations can be used to test the isomorphism between graphs. In particular, a card colouring is \emph{sound} when any two isomorphic graphs are assigned a colouring generating the coincident graph representations: $\forall G_1, G_2, G_1 \cong G_2 \implies c_{G_1} = c_{G_2}$. Sound colourings give us a sufficient condition for two graphs not to be isomorphic: whenever two graphs are assigned distinct representations, we can conclude they are not isomorphic. Given our interest in graph isomorphism testing, in the following we will always assume to work with sound colourings, even when not explicitly specified.

When colourings are defined on decks generated by the same selection policy, they can be compared by the notion of \emph{refinement}:
\begin{definition}
    Let $\pi$ be a subgraph selection policy and, $c, d$ be colourings over decks generated via $\pi$. We say that refines deck colouring $c$ \emph{refines} deck colouring $d$, if for all graphs $G_1$ and $G_2$, associated with decks $\mathcal{D}_1, \mathcal{D}_2$, and all cards $\mathcal{K} \in \mathcal{D}_1$ and $\mathcal{H} \in \mathcal{D}_2$ we have that $c^{\mathcal{D}_1}_\mathcal{K} = c^{\mathcal{D}_2}_\mathcal{H} \implies d^{\mathcal{D}_1}_\mathcal{K} = d^{\mathcal{D}_2}_\mathcal{H}$.
    We write $c \sqsubseteq d$.
\end{definition}
When both $c \sqsubseteq d$ and $d \sqsubseteq c$ hold, we say the two colourings are equivalent $c \equiv d$.

The notion of refinement is useful as we can compare deck-colourings in terms of their ability to disambiguate non-isomorphic graphs: whenever $c \sqsubseteq d$, if any two graphs are assigned equal deck-colouring by $c$, then they are also assigned equal deck-colouring by $d$. In other words, graphs which are indistinguishable by $c$ are also indistinguishable by $d$ and thus $d$ is ``at most as powerful'' as $c$ (in disambiguating between non-isomorphic graphs).

\todo[inline]{FF: the proof should be the same we have for node colourings in the MPSN paper}


Similar in the spirit of node-colour refinement algorithms, we can define card-colour refinement algorithms:
\begin{definition}
    Let $\pi$ be a subgraph selection policy and, $\mathcal{D} = \mathcal{S}_G^{\pi}$ be the deck generated by such policy over graph $G$. A card-colour refinement algorithm is a computable procedure which, given $\mathcal{D}$ as input, at any $t \in \mathbb{N}$ it outputs a deck colouring $c^{(t)}$ over $\mathcal{D}$ such that $c^{(t+1)} \sqsubseteq c^{(t)}$.
\end{definition}

Distinct card-colour refinement algorithms would differ in the way the deck-colouring is obtained, that is, in the way each card is assigned a colour at each time step $t \in \mathbb{N}$. Each card represents a subgraph, which is, effectively, a graph. Thus, a reasonable choice would be to use a node-colour refinement algorithm and to compute card colours as a function of the multiset of colours thereof. In order to correctly define a card-level algorithm leveraging on a node level one, we must ensure that a refinement at the level of node colours entails a refinement at the level of card colours. If card colours are obtained as an injection of the multiset of node colours, then a refinement at the level of node colours then this would be the case:
\begin{proposition}
    pass
\end{proposition}
\begin{proof}
    pass
\end{proof}

In the following, we term `encoder' the node-colour refinement algorithm that is employed to compute card colours. An implication of the Proposition above is that, given a pre-determined selection policy, the choice of the encoder determines the expressive power of the overall card-colour refinement algorithm.
\begin{corollary}
    say that given two encoders such that the first refines the second, under the same policy we have that the deck colouring associated to the former refines the latter
\end{corollary}

Example here: same policy with 1-WL vs. 3-WL encoders.

\todo[inline]{FF: Question: what happens if an encoder is \emph{strictly} more expressive than another?}


